Quantum-Gated Task-interaction Knowledge Distillation for Pre-trained Model-based Class-Incremental Learning

Class-incremental learning (CIL) aims to continuously accumulate knowledge from a stream of tasks and construct a unified classifier over all seen classes. Although pretrained models (PTMs) have shown promising performance in CIL, they still struggle with the entanglement of multi-task subspaces, leading to catastrophic forgetting when task routing parameters are poorly calibrated or task-level representations are rigidly fixed. To address this issue, we propose a novel Quantum-Gated Task-interaction Knowledge Distillation (QKD) framework that leverages quantum gating to guide inter-task knowledge transfer. Specifically, we introduce a quantum-gated task modulation gating mechanism to model the relational dependencies among task embedding, dynamically capturing the sample-to-task relevance for both joint training and inference across streaming tasks. Guided by the quantum gating outputs, we perform task-interaction knowledge distillation guided by these task-embedding-level correlation weights from old to new adapters, enabling the model to bridge the representation gaps between independent task subspaces. Extensive experiments demonstrate that QKD effectively mitigates forgetting and achieves state-of-the-art performance.

==> subtex/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Recent advances in deep learning have driven remarkable progress across a wide range of real-world applications, accelerating the digital transformation of both emerging and traditional domains~\cite{IAI_1,IAI_2}. However, in the real world, data is streaming, non-stationary, and exponentially growing, which raises a fundamental question:\textit{ how can an intelligent system continuously learn from an ever-evolving data stream with finite computational resources?} To address this challenge, continual learning (also known as incremental learning) aims to endow deep neural networks with the ability to learn new tasks sequentially while retaining knowledge of previously learned tasks~\cite{Continualsurvey}. Within this paradigm, class-incremental learning (CIL) focuses on building a unified classifier over all seen classes~\cite{CILsurvey}. A central difficulty arises because the task boundaries are explicit during training but ambiguous during inference, leading to subspace entanglement among tasks. Such entanglement exacerbates catastrophic forgetting, as the model may confuse representations of different tasks when task identity is unknown in inference.

With the rise of pretrained models (PTMs), recent CIL methods have leveraged parameter-efficient fine-tuning (PEFT) techniques—such as prompt and adapter tuning—to adapt frozen backbones to downstream incremental tasks~\cite{PTMsurveyCIL}. Prompt-based approaches typically maintain a global prompt pool containing multiple key–prompt pairs. Each input sample retrieves the most relevant prompt via similarity matching on its embedding from the frozen backbone~\cite{l2p,dualprompt,codaprompt}. While this method implicitly enables a degree of task sharing and task-specific specialization, it suffers from blind selection and potential prompt overwriting, leading to unstable task adaptation. In contrast, adapter-based methods allocate an independent adapter per task, which effectively isolates task-specific learning and prevents interference~\cite{EASE,li2025mote}. However, this design fails to capture cross-task correlations and struggles when task-specific feature subspaces overlap. During inference, the model may incorrectly route samples to unrelated adapters, causing performance degradation. These limitations motivate a key question: \textit{Is it possible to explicitly model the correlation between an input sample and all existing task modules, and use this relational information to guide both new module training and multi-adapter inference?}

To this end, we propose a Quantum-Gated Knowledge Distillation (QKD) framework for PTM-based class-incremental learning. Following prior works~\cite{EASE,li2025mote}, we freeze the pretrained backbone and allocate a new adapter for each incremental task. To explicitly model the interaction between incoming samples and all previously learned tasks, we design a mutual-information-modulated quantum gating mechanism. Concretely, we construct a lightweight quantum circuit that takes as input the task-level embeddings obtained from the pretrained model after the first task. These embeddings are encoded into quantum states, where the interference patterns between states reflect the correlation strength between the current sample and each learned task. The quantum gate outputs soft routing coefficients that dynamically weight the contribution of each adapter. During training, these quantum-derived coefficients guide a correlation-weighted feature-level knowledge distillation process, enabling the new adapter to absorb informative knowledge from prior adapters in proportion to their relevance. This promotes inter-task representation sharing and mitigates feature subspace entanglement.
During inference, the same quantum gate performs adaptive routing among adapters, allowing the model to leverage historical knowledge without confusing task-specific representations. Through this unified quantum-gated design, QKD achieves more stable task interaction, better subspace calibration, and enhanced resistance to catastrophic forgetting.

To evaluate the effectiveness of our proposed framework, we conducted extensive experiments on five widely used benchmark datasets — CIFAR-100~\cite{CIFAR}, CUB-200~\cite{CUB}, ImageNet-A~\cite{ImageNetA}, ImageNet-R~\cite{ImageNetR}, and VTAB~\cite{VTAB} — under various incremental learning settings.
Across five standard evaluation protocols for class-incremental learning, our method consistently outperforms the second-best approach by 1$\%$, 2$\%$, 3$\%$, 4$\%$, and 5$\%$, respectively, demonstrating its superior generalization and robustness.

Our main contributions can be summarized as follows: (1) We are the first to integrate quantum machine learning into class-incremental learning, introducing a mutual-information-modulated quantum gating mechanism that explicitly models the relational dependencies between samples and task-specific representations; (2) Correlation-Weighted Multi-Adapter Knowledge Distillation. Based on the task correlation estimated by the quantum gate, we perform correlation-weighted, feature-level knowledge distillation across adapters, effectively bridging the representational gap between disjoint task subspaces. (3)Extensive experiments verify that our approach achieves state-of-the-art performance across multiple benchmarks. Moreover, our findings highlight the potential and significance of quantum learning paradigms in advancing continual and incremental learning research.
